Readout Technologies for Future Detectors

It is essential to develop novel cost-effective readout technologies to maximize the discovery potential of future HEP experiments.

==> Exec.tex <==
\section{Executive Summary}
\label{s.exec} 



==> Technologies/MultiplexTech.tex <==
\subsection{Multiplex High-speed Readout}
A different architecture is to use Wavelength Division Multiplexing (WDM), where no bit rate up-conversion
is needed, and it is possible to collect data from distant modules onto the the same fiber. One example, based on SBIR-supported development by Freedom Photonics, LLC, all complex electronics are outside the radiation environment and only modulators on silicon photonic chips must reside in the detector volume. Furthermore, this method does not require a specific bit rate or synchronization for the signals to be multiplexed, even allowing signals with different bit rates to be combined on the same fiber. The footprint and power in the radiation environment are small, as there is no ASIC needed inside the detector. There is no hard limit on the number of signals that can multiplexed onto one fiber, permitting evolution to ever higher bandwidth detectors.
\begin{figure}[tbp]
\begin{center}
\includegraphics[width=0.8\textwidth]{Technologies/Figures/WDM_RRM.pdf}
\caption{WDM readout system proposed architecture. RRM stands for Ring Resonator Modulator\label{fig:WDM_RRM}.}
\end{center}
\end{figure}
The proposed concept is shown in Fig~\ref{fig:WDM_RRM}. Multiple laser wavelengths are combined onto a single fiber off-detector. Each wavelength is a CW (Continuous Wave) carrier that will be modulated on-detector using a ring resonator. While Current technology is already demonstrating 20Mbps modulation, the radiation hard data sources (detector front end chips) are expected to remain at the 1Gbps level, as this simplifies radiation tolerant design, and a typical detector consists of many “low” bandwidth sources rather than few high bandwidth ones. The off-detector tunable laser sources can be commercial grade and already exist: a picture of a Freedom Photonics tunable source is shown in the figure. The on-detector amplitude modulation is carried out by Ring Resonator Modulators (RRM) on a photonic chip. These must be radiation hard,
and such technology is being developed with SBIR and other support. The electrical drivers to feed the RRM’s are analog circuits that can be separate CMOS chips or possibly integrated into the detector readout chips. As RRMs are also implemented in a (silicon photonic) CMOS process, there is also potential to integrate drivers and RRM’s on the same chip, further reducing mass, complexity, and cost, while increasing performance. Commercial demodulating technology (off-detector) also exists. The Fig. 1 concept includes distant detector elements multiplexed onto the same fiber. This would allow a macro-assembly to have just one input and one output fibers, with the total bandwidth required dictating how many laser frequencies are needed. Each RRM works at a specific wavelength, but that wavelength can drift, for example due to temperature. The incoming wavelength must track these shifts, so a feedback mechanism is needed. The architecture allows for this by monitoring the return signals on the output fiber. The feedback can be implemented either by adjusting the laser wavelength or by acting on the RRM (for example with a heater). The method used will depend on practical considerations of a given implementation. The WDM readout architecture proposed here will enable higher bandwidth, lower mass, highly scalable readout of future tracking detectors.

==> ack.tex <==
\section{Acknowledgements}

We gratefully acknowledge for their advice and careful reading of this report.

